Sign Gradient Descent-based Neuronal Dynamics: ANN-to-SNN Conversion Beyond ReLU Network

Spiking neural network (SNN) is studied in multidisciplinary domains to (i) enable order-of-magnitudes energy-efficient AI inference and (ii) computationally simulate neuro-scientific mechanisms. The lack of discrete theory obstructs the practical application of SNN by limiting its performance and nonlinearity support. We present a new optimization-theoretic perspective of the discrete dynamics of spiking neurons. We prove that a discrete dynamical system of simple integrate-and-fire models approximates the sub-gradient method over unconstrained optimization problems. We practically extend our theory to introduce a novel sign gradient descent (signGD)-based neuronal dynamics that can (i) approximate diverse nonlinearities beyond ReLU and (ii) advance ANN-to-SNN conversion performance in low time steps. Experiments on large-scale datasets show that our technique achieves (i) state-of-the-art performance in ANN-to-SNN conversion and (ii) is the first to convert new DNN architectures, e.g., ConvNext, MLP-Mixer, and ResMLP. We publicly share our source code at https://github.com/snuhcs/snn_signgd .

==> icml2024/proofs/integrate_and_fire_rate.tex <==
\begin{proof} 
Rearranging the membrane equation for $u_{pre}$,
\begin{equation}
u_{pre}(t+1) = u_{pre}(t) - \theta_{th} s(t) + RI(t+1)
\end{equation}
Spike mechanism links the recurrence relation of the membrane potential $u_{pre}$ and rate-coded output $y$ as follows.
\begin{align*}
    s(t) &=  ty(t) - (t-1)y(t-1)\\
    &= \frac{-1}{\theta_{th}} (u_{pre}(t+1) - u_{pre}(t) - RI(t+1)) 
\end{align*}
Solving the recurrence relation of $y$ and $u_{pre}$ yields a linear relation of membrane potential, input and output activations. 
\begin{equation}
\label{eq:linear_mempot_output}
ty(t) = \frac{-1}{\theta_{th}} (u_{pre}(t+1) - u(0) - R(t+1) \tilde{x}(t+1))
\end{equation}
With~\eqref{eq:linear_mempot_output}, we reduce the rate coding equation~\eqref{eq:rate} into a discrete dynamical system of $y$ and $\tilde{x}$.
\begin{align*}
    y(t) &= \frac{t-1}{t} y(t-1) \\
    &+ \frac{1}{t} \mathbb{H} (R t\tilde{x}(t)-\theta_{th} (t-1)y(t-1) 
    + u(0) - \theta_{th})
\end{align*}
From this equation, we substitute $y(t)$ with the $\tilde{f}(t)$ (Eq.~\ref{eq:main_if_tthapprox})  and use the scale-invariance of step function $\mathbb{H}$ to obtain
\begin{align*}
    &\tilde{f}(t) = \frac{t}{t+1} \tilde{f}(t-1) + \mathbb{H}(Rt\tilde{x}(t) - \theta_{th}t\tilde{f}(t-1))\\
  &= \tilde{f}(t-1) - \frac{1}{t+1} (\tilde{f}(t-1) - \mathbb{H}(\frac{R}{\theta_{th}}\tilde{x}(t) - \tilde{f}(t-1)))\\
  &= \tilde{f}(t-1) - \frac{1}{t+1} \nabla_{y}\mathcal{L}(\tilde{f}(t-1); \tilde{x}(t))
\end{align*}
This corresponds to the subgradient method with a diminishing learning rate inverse proportional to the time. 
The objective function $\mathcal{L}(y;x)$ is a convex $l^2$-regularized negative ReLU function. Its minimizer is $\text{ReLU1}(\frac{R}{\theta_{th}} x)$.
\end{proof}

==> icml2024/theorems/corollary_signgd/gelu.tex <==
\begin{corollary}
\label{cor:gelu_signsgd}
Let $g(x) = \frac{x}{1+e^{-1.702x}}$ be the sigmoid approximation of GELU function~\cite{hendrycks2016gelu}. SignGD (Eq.~\ref{eq:main_signsgd_subg}) with $\mathcal{L}(y;x) = \frac{1}{2}\Vert y - g(x) \Vert^2$ is equivalent to the signGD-based neuronal dynamics~(Def.~\ref{def:signgd_dynamics})
satisfying Eq.~\ref{eq:main_signsgd_coeff_condition}, $\eta(t) = \alpha_2(t) = \beta_2(t)$ and ~$s(t) = \mathbb{H}\big((1 + (e^{-1.702})^{v(t)}) u(t) - \beta_1(t) v(t) \big)$ (Proof at~\ref{thm:signgd_gelu})
\iffalse
\begin{equation*}
\begin{split}
s(t) =& \mathbb{H}\big((1 + (e^{-1.702})^{v(t)}) u(t) - \beta_1(t) v(t) \big) 
\end{split}
\end{equation*}  
\fi
\end{corollary}

==> icml2024/theorems/corollary_signgd/leakyrelu.tex <==
\begin{corollary}
\label{cor:leakyrelu_signsgd}
SignGD (Eq.~\ref{eq:main_signsgd_subg}) with $\mathcal{L}(y;x) = \frac{1}{2}\Vert y - \text{LeakyReLU(x, $\delta$)} \Vert^2$, where $\delta$ is the negative slope, is equivalent to the signGD-based neuronal dynamics~(Def.~\ref{def:signgd_dynamics})
satisfying Eq.~\ref{eq:main_signsgd_coeff_condition}, $\alpha_2(t) = \beta_2(t)$ and (Proof at~\ref{thm:signgd_leakyrelu})
\begin{equation*}
\begin{split}
s(t) =~& \mathbb{H}(v(t))\mathbb{H}\big(u(t) -\beta_1(t)v(t)\big) \\
&+ \mathbb{H}(-v(t))\mathbb{H}\big(u(t) - \delta \beta_1(t)v(t)\big) 
\end{split}
\end{equation*}    
\end{corollary}

==> icml2024/theorems/corollary_signgd/relu.tex <==
\begin{corollary}
\label{cor:relu_signsgd}
SignGD (Eq.~\ref{eq:main_signsgd_subg}) with $\mathcal{L}(y;x) = \frac{1}{2}\Vert y - \text{ReLU(x)} \Vert^2$ is equivalent to the signGD-based neuronal dynamics~(Def.~\ref{def:signgd_dynamics}) satisfying Eq.~\ref{eq:main_signsgd_coeff_condition}, $\alpha_2(t) = \beta_2(t)$ and $s(t) = \mathbb{H}\big(v(t)\big)\mathbb{H}\big(u(t) - \beta_1(t)v(t)\big) + \mathbb{H}\big(-v(t)\big)\mathbb{H}\big(u(t)\big) $
\iffalse
\begin{equation*}
\begin{split}
s(t) =& \mathbb{H}\big(v(t)\big)\mathbb{H}\big(u(t) - \beta_1(t)v(t)\big) + \mathbb{H}\big(-v(t)\big)\mathbb{H}\big(u(t)\big) 
\end{split}
\end{equation*}
\fi
\end{corollary}
